ChatDB: Augmenting LLMs with Databases as Their Symbolic Memory

Large language models (LLMs) with memory are computationally universal. However, mainstream LLMs are not taking full advantage of memory, and the designs are heavily influenced by biological brains. Due to their approximate nature and proneness to the accumulation of errors, conventional neural memory mechanisms cannot support LLMs to simulate complex reasoning. In this paper, we seek inspiration from modern computer architectures to augment LLMs with symbolic memory for complex multi-hop reasoning. Such a symbolic memory framework is instantiated as an LLM and a set of SQL databases, where the LLM generates SQL instructions to manipulate the SQL databases. We validate the effectiveness of the proposed memory framework on a synthetic dataset requiring complex reasoning. The project website is available at https://chatdatabase.github.io/ .

==> tables/structure_output.tex <==
 \begin{figure*}[p]
    \scriptsize
    \centering
    \begin{tabular}{@{}p{0.475\columnwidth}p{0.475\columnwidth}@{}}
    \toprule
    \textbf{(a) Purchasing goods: the shop purchases goods from suppliers.} 

    \rule[1.2ex]{0.475\columnwidth}{0.4pt}
    
    \textbf{Record:}
    \textcolor[HTML]{3078BE}
    {\textbf{We restocked our store on 2023-01-01 with a new supply of fruits from `ABC' (abc\_sup@example.com, 10080). The purchased quantities include 24 kg cherry, at unit prices of 0.8. Our intended selling price of cherry is 1.3 dollars per unit.}
    }
    
    \textbf{ChatDB:}
    
    Begin to interact with the external database (symbolic memory).

    Step1: Insert supplier `ABC' if not exists
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO suppliers (supplier_name, contact_number, email)
SELECT 'ABC', '10080', 'abc_sup@example.com'
WHERE NOT EXISTS (SELECT 1 FROM suppliers WHERE supplier_name = 'ABC');
    \end{minted}
    % Database response: insert data successfully.

    Step2: Insert fruit (set the selling price to NULL and stock quantity to 0) if not exists
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO fruits (fruit_name, selling_price, stock_quantity, fruit_type, shelf_life)
SELECT 'cherry', NULL, 0, NULL, NULL
WHERE NOT EXISTS (SELECT 1 FROM fruits WHERE fruit_name = 'cherry');
    \end{minted}

    Step3: Insert purchase
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO purchases (supplier_id, purchase_date, total_cost)
VALUES ((SELECT supplier_id FROM suppliers WHERE supplier_name = 'ABC'), '2023-01-01', 24 * 0.8);
    \end{minted}

    Step4: Insert purchase item
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO purchase_items (purchase_id, fruit_id, quantity_purchased, cost_per_item, item_total_cost)
VALUES ((SELECT MAX(purchase_id) FROM purchases), (SELECT fruit_id FROM fruits WHERE fruit_name = 'cherry'), 24, 0.8, 24 * 0.8);
    \end{minted}

    Step5: Update the stock quantity of cherry
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
UPDATE fruits 
SET stock_quantity = stock_quantity + 24
WHERE fruit_name = 'cherry';
    \end{minted}

    Step6: Update the selling price of cherry if given new selling price
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
UPDATE fruits 
SET selling_price = 1.3
WHERE fruit_name = 'cherry';
    \end{minted}

    
    &    
    \textbf{(b) Selling goods: customers buy goods from the shop}

    \rule[1.2ex]{0.475\columnwidth}{0.4pt}
    
    \textbf{Record:}
    \textcolor[HTML]{3078BE}
    {\textbf{A sale was made on 2023-01-02 to `Bob Smith' (contact details: 123-456-7893, bob.smith@example.com). The items purchased were 9 kg apple, 4 kg cherry.}}
    
    \textbf{ChatDB:}
    
    Begin to interact with the external database (symbolic memory).

    Step1: Insert customer 'Bob Smith' if not exists
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO customers (first_name, last_name, phone_number, email)
SELECT 'Bob', 'Smith', '123-456-7893', 'bob.smith@example.com'
WHERE NOT EXISTS (SELECT 1 FROM customers WHERE phone_number = '123-456-7893');
    \end{minted}

    Step2: Insert sale
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO sales (customer_id, sale_date, total_price)
VALUES ((SELECT customer_id FROM customers WHERE phone_number = '123-456-7893'), '2023-01-02', (SELECT selling_price FROM fruits WHERE fruit_name = 'apple') * 9 + (SELECT selling_price FROM fruits WHERE fruit_name = 'cherry') * 4);
    \end{minted}

    Step3: Insert sale item
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
INSERT INTO sale_items (sale_id, fruit_id, quantity_sold, price_per_item, item_total_price)
VALUES ((SELECT MAX(sale_id) FROM sales), (SELECT fruit_id FROM fruits WHERE fruit_name = 'apple'), 9, (SELECT selling_price FROM fruits WHERE fruit_name = 'apple'), (SELECT selling_price FROM fruits WHERE fruit_name = 'apple') * 9),
((SELECT MAX(sale_id) FROM sales), (SELECT fruit_id FROM fruits WHERE fruit_name = 'cherry'), 4, (SELECT selling_price FROM fruits WHERE fruit_name = 'cherry'), (SELECT selling_price FROM fruits WHERE fruit_name = 'cherry') * 4);
    \end{minted}

    Step4: Update the stock quantity of apple and cherry
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
UPDATE fruits 
SET stock_quantity = CASE 
    WHEN fruit_name = 'apple' THEN stock_quantity - 9
    WHEN fruit_name = 'cherry' THEN stock_quantity - 4
    ELSE stock_quantity
END
WHERE fruit_name IN ('apple', 'cherry');
    \end{minted}
    
    \\
    \midrule
    \textbf{(c) Return of goods: customers bring back purchased items to the shop.}

    \rule[1.2ex]{0.475\columnwidth}{0.4pt}

    \textbf{Record:}
    \textcolor[HTML]{3078BE}
    {\textbf{Because the customer returned their purchase, we are required to undo the sales transaction made by customer `John Doe' (phone: 123-456-7890, email: john.doe@example.com) on 2023-01-05.}}
    
    \textbf{ChatDB:}
    
    Begin to interact with the external database (symbolic memory).

    Step1: Find the sale\_id for this customer on this date
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
SELECT sale_id FROM sales 
WHERE customer_id = (SELECT customer_id FROM customers WHERE phone_number = '123-456-7890' AND email = 'john.doe@example.com') AND sale_date = '2023-01-05';
    \end{minted}
    Database response:
    \begin{minted}[fontsize=\tiny, breaklines]{python}
+---------+
| sale_id |
+---------+
|    9    |
+---------+
    \end{minted}

    Step2: Get all the fruit\_id and quantity\_sold for this sale, replace \textless sale\_id\textgreater \ with the results from the previous queries
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
SELECT fruit_id, quantity_sold FROM sale_items 
WHERE sale_id = 9 [<sale_id>];
    \end{minted}
        Database response:
    \begin{minted}[fontsize=\tiny, breaklines]{python}
+----------+---------------+
| fruit_id | quantity_sold |
+----------+---------------+
|    7     |       10      |
|    6     |        9      |
+----------+---------------+
    \end{minted}

    &
    
    Step3: Increase the stock\_quantity for each fruit sold in this sale, replace \textless quantity\_sold\textgreater \  \textless fruit\_id\textgreater \ with the results from the previous queries
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
UPDATE fruits
SET stock_quantity = stock_quantity + 10 [<quantity_sold>]
WHERE fruit_id = 7 [<fruit_id>];

UPDATE fruits
SET stock_quantity = stock_quantity + 9 [<quantity_sold>]
WHERE fruit_id = 6 [<fruit_id>];
    \end{minted}

    Step4: Delete the sale items for this sale, replace \textless sale\_id\textgreater \ with the results from the previous queries
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
DELETE FROM sale_items WHERE sale_id = 9 [<sale_id>];
    \end{minted}

    Step5: Delete the sale record, replace \textless sale\_id\textgreater \ with the results from the previous queries
    \begin{minted}[fontsize=\tiny, breaklines]{sql}
DELETE FROM sales WHERE sale_id = 9 [<sale_id>];
    \end{minted}
    
    \rule[0ex]{0.475\columnwidth}{0.4pt}
    
     
    \textbf{(d) Changing price: modify the price of the goods.}

    \rule[1.2ex]{0.475\columnwidth}{0.4pt}

    \textbf{Record:}
    \textcolor[HTML]{3078BE}
    {\textbf{On 2023-01-05, the sale price of pear in the store was changed to 1.6 dollar per unit.}}
    
    \textbf{ChatDB:}
    
    Begin to interact with the external database (symbolic memory).

    Step1: Update the selling price of pear
    \begin{minted}[fontsize=\tiny, breaklines]{sql}   
UPDATE fruits 
SET selling_price = 1.6
WHERE fruit_name = 'pear';
    \end{minted}

     \\
    \bottomrule
    \end{tabular}
    \caption{Model outputs from test prompts that ask the model to generate according to specified structures. The gray ellipsis \textcolor[HTML]{808080}{[...]} indicates that the response was trimmed to fit this page, but the generated text is actually longer.}
    \label{fig:four_manipulations}
    
\end{figure*}

==> tables/tab_overview.tex <==
\begingroup
\setlength{\tabcolsep}{3pt}
\begin{table}[!t]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
                & Verification & Format  & Culture & Scaling   \\ \midrule
General Purpose &      \score{1}{3}      &    \score{2}{3}     &   \score{2}{3}      & \score{3}{3} \\
Academic Exams  & \score{2}{3}    & \score{2}{3} &   \score{2}{3}      &    \score{2}{3}     \\
Value Alignment &  \score{1}{3}   &  \score{1}{3}     & \score{3}{3} &      \score{1}{3}   \\
Counterfactual &  \score{2}{3}   & \score{1}{3}      &     \score{1}{3}    &    \score{2}{3}     \\
Code            & \score{3}{3}    & \score{3}{3}&     \score{1}{3}    & \score{2}{3} \\ \bottomrule
\end{tabular}%
}
\caption{The four dimensions we consider when constructing COIG instruction following data. \textbf{Verification}: whether the response can be verified. \textbf{Format}: whether the format is crucial. \textbf{Culture}: whether the response will depend on a certain culture. \textbf{Scale}: whether scaling is important. The number of filled stars presents the importance of a certain factor.}
\label{tab:overview}
\end{table}
\endgroup{}
